An Institutional Framework for Heterogeneous Formal Development in UML

We present a framework for formal software development with UML. In contrast to previous approaches that equip UML with a formal semantics, we follow an institution based heterogeneous approach. This can express suitable formal semantics of the different UML diagram types directly, without the need to map everything to one specific formalism (let it be first-order logic or graph grammars). We show how different aspects of the formal development process can be coherently formalised, ranging from requirements over design and Hoare-style conditions on code to the implementation itself. The framework can be used to verify consistency of different UML diagrams both horizontally (e.g., consistency among various requirements) as well as vertically (e.g., correctness of design or implementation w.r.t. the requirements).

==> preamble.tex <==
\usepackage{xspace,calc}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage{times}
\usepackage[scaled=.85]{helvet}
\usepackage{babel}
\makeatletter\let\proof\@undefined\let\endproof\@undefined\makeatother%
\usepackage{amsmath,amssymb,amsthm,stmaryrd,mathrsfs}
\makeatletter\let\mathmargin\@mathmargin\makeatother
\usepackage{rotating}
\usepackage{xspace}
\usepackage{url}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{tikz}
\usetikzlibrary{matrix,shapes,arrows,calc}
\usepackage{enumitem}
\usepackage{float}
\usepackage{subfigure}
\usepackage{listings}
\lstset{%
  language=C,
  basicstyle=\ttfamily, %\fontsize{8pt}{8pt}\selectfont, % Standardschrift
  numbers=none,               % Ort der Zeilennummern
  numberstyle=\fontsize{6pt}{6pt}\selectfont,          % Stil der Zeilennummern
  %stepnumber=2,               % Abstand zwischen den Zeilennummern
  numbersep=7pt,              % Abstand der Nummern zum Text
  tabsize=4,                  % Groesse von Tabs
  extendedchars=true,         %
  breaklines=true,            % Zeilen werden Umgebrochen
  numberbychapter=false,
  %keywordstyle=\color{red},      
  %keywordstyle=[1]\textbf,    % Stil der Keywords
  %keywordstyle=[2]\textbf,    %
  %keywordstyle=[3]\textbf,    %
  %keywordstyle=[4]\textbf,   \sqrt{\sqrt{}} % 
  %stringstyle=\color{white}\ttfamily, % Farbe der String
  showspaces=false,           % Leerzeichen anzeigen ?
  showtabs=false,             % Tabs anzeigen ?
  captionpos=b,
  %frame=tb,
  xleftmargin=17pt,
  framexleftmargin=17pt,
  framexrightmargin=5pt,
  framexbottommargin=4pt,
  %backgroundcolor=\color{lightgray},
  showstringspaces=false,      % Leerzeichen in Strings anzeigen ?  
  escapeinside={(*@}{@*)},
  keywordsprefix={.},
}
% \usepackage[backend=biber,
%             style=llncs,
%             defernumbers=true,
%             firstinits=true,
%             maxnames=999,minnames=4,
%             isbn=false,doi=false,eprint=false]{biblatex}

\def\powerset{\wp}
\def\NZ{\mathbb{N}}
\def\ZZ{\mathbb{Z}}
\def\BZ{\mathbb{B}}
\def\RZ{\mathbb{R}}
\def\Rho{\mathit{P}}
\newcommand{\Eta}{H}
\newcommand{\Tau}{\mathit{T}}
\newcommand{\Ypsilon}{\mathit{Y}}
\newcommand{\omikron}{\ensuremath{o}}
\newcommand{\partialto}{\rightharpoonup}
\def\iff{\mathrel{\Leftrightarrow}}
\def\divop{\mathbin{\mathrm{div}}}
\def\modop{\mathbin{\mathrm{mod}}}
\def\im{\mathop{\mathrm{im}}}
\def\pll{\mathrel{\|}}
\def\fibop{\mathop{\mathrm{fib}}\nolimits}
\def\trueval{\mathit{tt}}
\def\falseval{\mathit{ff}}
\def\dom{\mathrm{dom}}
\def\infers{\mathrel{\vdash}}
\def\iteop{\mathrm{ite}}
\def\idop{\mathrm{id}}
\def\bottom{\bot}
\def\dbottom{\mathnormal{\bot\!\!\!\bot}}
\def\limp{\mathrel{\Rightarrow}}
\def\chooserel{\mathrel{\varepsilon}}
\def\lequiv{\mathrel{\Leftrightarrow}}
\def\partto{\mathrel{\rightharpoonup}}
\def\isorel{\mathrel{\cong}}
\def\sem#1{\mathopen\llbracket#1\mathclose\rrbracket}
\def\restrictop{\mathnormal{\upharpoonright}}
\def\preimop{{}^\bullet}
\def\compfun{\mathbin{\circ}}
\def\comprel{\mathbin{\circ}}
\def\isorel{\mathrel{\cong}}
\def\angleplus{\mathbin{\langle\!{+}\!\rangle}}
\def\fixop{\mathop{\smash{\mathbf{Y}}}\nolimits}
\def\applyop{\mathop{\mathrm{apply}}\nolimits}
\def\curryop{\mathop{\mathrm{curry}}\nolimits}
\newcommand{\structrule}[2]{\dfrac{%
\renewcommand{\arraystretch}{1.1}%
\begin{array}{@{}c@{}}#1\end{array}}{%
\renewcommand{\arraystretch}{1.1}%
\begin{array}{@{}l@{}}#2\end{array}}\vspace{3pt}}
\def\shows{\mathrel{\Vdash}}
\def\diverges{\mathnormal{\uparrow}}
\def\finop{\mathnormal{\mathscr{K}}}
\DeclareMathOperator{\colim}{\mathrm{colim}}
%\def\colim{\mathop{\mathrm{colim}}}
\def\invlim{\mathop{\underleftarrow{\lim}}}
\def\initdom{\emptyset_{\bottom}}
\def\xrightleftarrows#1#2{\mathrel{\raisebox{-.2ex}{$\begin{array}{@{}c@{}}\xrightarrow{#1}\\[-1.5ex]\xleftarrow[#2]{}\end{array}$}}}
\def\inclop{\hookrightarrow}

\def\IMP{{\textbf{IMP}}\xspace}
\def\syncat#1{{\normalfont\textrm{#1}}}
\def\semcat#1{{\normalfont\mathit{#1}}}
\newcommand{\code}[1]{\normalfont\texttt{\spaceskip=3pt\frenchspacing\def\{{\char123}\def\}{\char125}\def\^{\char94}\def\_{\char95}#1}}

\def\State{\Sigma}

\def\numsem#1{\mathop{\mathcal{N}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}
\def\boolsem#1{\mathop{\mathcal{B}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}
\def\arithsem#1{\mathop{\mathcal{A}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}

\def\nstrans{\mathrel{\rightarrow}}
\def\fvar{\mathop{\mathrm{fvar}}}
\def\floc{\mathop{\mathrm{fvar}}\nolimits_L}
\def\stateop{\mathop{\mathit{state}}}
\def\dvar{\mathop{\mathrm{dvar}}}
\def\updvarop{\mathop{\mathit{upd}}\nolimits_V}
\def\updprocop{\mathop{\mathit{upd}}\nolimits_P}
\def\newop{\mathop{\mathit{new}}}

\def\sostrans{\mathrel{\Rightarrow}}

\def\refsem#1{\mathop{\mathcal{R}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}

\def\stmsem#1{\mathop{\mathcal{S}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}
\def\contstmsem#1{\mathop{\mathcal{C}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}

\def\ASSN{{\textbf{ASSN}}\xspace}
\def\termsem#1{\mathop{\mathcal{T}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}
\def\frmsem#1{\mathop{\mathcal{F}\mathopen\llbracket#1\mathclose\rrbracket}\nolimits}
\def\phoare#1#2#3{\{ #1 \}\,#2\,\{ #3 \}}
\def\thoare#1#2#3{[ #1 ]\,#2\,[ #3 ]}
\def\flog{\mathop{\mathrm{flog}}}
\def\extop{\mathop{\mathrm{ext}}\nolimits}
\def\wpop{\mathop{\mathrm{wp}}\nolimits}
\def\wlpop{\mathop{\mathrm{wlp}}\nolimits}

% Literals
\newcommand{\clop}[1]{\syntax{\{}{#1}\syntax{\}}}

% Types
\newcommand{\ptop}[1]{\syntax{(}{#1}\syntax{)}}
\DeclareMathOperator{\typeop}{\mathit{type}}
\DeclareMathOperator{\baseop}{\mathit{base}}

% Type inference
\DeclareMathOperator{\fdop}{\mathit{fd}}
\newcommand{\entails}{\mathrel{\vdash}}
\newcommand{\annotated}{\mathrel{\triangleright}}

% Operational semantics
\DeclareMathOperator{\acttypeop}{\mathit{actual}}
\DeclareMathOperator{\flattenop}{\mathit{flatten}}
\DeclareMathOperator{\makeop}{\mathit{make}}
\DeclareMathOperator{\attrop}{\mathit{attr}}
\DeclareMathOperator{\methop}{\mathit{meth}}
\DeclareMathOperator{\implop}{\mathit{impl}}
\newcommand{\ordersrel}{\mathrel{\leadsto}}
\newcommand{\evalsto}{\mathrel{\downarrow}}

% Denotational semantics
\DeclareMathOperator{\evalop}{\mathit{eval}}
\DeclareMathOperator{\liftop}{\mathit{lift}}
\DeclareMathOperator{\oliftop}{\overline{\mathit{lift}}}
\DeclareMathOperator{\condop}{\mathit{cond}}
\DeclareMathOperator{\iterateop}{\mathit{iterate}}
\DeclareMathOperator{\sigop}{\mathit{sig}}

\newcommand{\Sig}[1]{\text{$#1$-$\mathrm{Sig}$}}
\newcommand{\Str}[1]{\text{$#1$-$\mathrm{Str}$}}
\newcommand{\trans}{\mathrel{\to}}
\def\reductop{\mathnormal{|}}
\def\natto{\mathrel{\dot{\mathnormal{\to}}}}

\newcommand{\opop}{\mathrm{op}}
\newcommand{\op}{^{\opop}}
\newcommand{\grothop}{\mathcal{G}}
\newcommand{\grothpair}[2]{\langle #1, #2\rangle}
\newcommand{\grothreduct}[3]{#1\reductop_{#2}#3}
\newcommand{\grothforward}[3]{#1^{\reductop_{#2}#3}}

\newcommand{\osSig}{\mathit{Sig}^{\leq}}
\newcommand{\osStr}{\mathit{Str}^{\leq}}
\newcommand{\osVal}{\mathit{\!Val}^{\leq}}
\newcommand{\osU}{U^{\leq}}
\newcommand{\osK}{\mathscr{T}^{\leq}}

\newcommand{\semtruth}{\mathnormal{\ast}}

%% UML
\newcommand{\uml}[1]{\textsf{#1}}
\newcommand{\stereotype}[1]{\uml{\flqq#1\frqq}}
\newcommand{\aggregation}{\raisebox{0.2pt}{\begin{sideways}\fontsize{6pt}{6pt}\selectfont$\lozenge$\end{sideways}}}
\newcommand{\composition}{\raisebox{0.2pt}{\begin{sideways}\fontsize{6pt}{6pt}\selectfont$\blacklozenge$\end{sideways}}}

\DeclareMathAlphabet{\mathsfsl}{OT1}{cmss}{m}{sl}

\newcommand{\FOL}{\text{\textit{FOL$^{=}$}}\xspace}
\newcommand{\PFOL}{\text{\textit{PFOL$^{=}$}}\xspace}
\newcommand{\PCFOL}{\text{\textit{PCFOL$^{=}$}}\xspace}
\newcommand{\SubPFOL}{\text{\textit{SubPFOL$^{=}$}}\xspace}
\newcommand{\SubPCFOL}{\text{\textit{SubPCFOL$^{=}$}}\xspace}
\newcommand{\ResSubPCFOL}{\text{\textit{ResSubPCFOL$^{=}$}}\xspace}

\newcommand{\angles}[1]{\langle #1 \rangle}


%% From MPhil
\newcommand{\category}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\functor}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\functorsymbol}[1]{#1}

\newcommand{\ModReduct}{\ensuremath{\category{Mod\_Reduct}}\xspace}

% These are institution functors
\newcommand{\Sen}{\functor{sen}}
\newcommand{\ModFunctor}{\functor{mod}}

% these are (projection) functions
%\newcommand{\Sig}{\ensuremath{\mathop{\text{\textbf{Sig}}}}}
\newcommand{\Mod}{\ensuremath{\mathop{\text{\textbf{Mod}}}}}
\newcommand{\Axioms}{\ensuremath{\mathop{\text{\textbf{Ax}}}}}
\newcommand{\flatten}{\ensuremath{\mathop{\text{\textit{flatten}}}}}
\newcommand{\LHS}{L.H.S\xspace}
\newcommand{\RHS}{R.H.S\xspace}
\newcommand{\Isabelle}{Isabelle\xspace}
\newcommand{\IsabelleHOL}{Isabelle/HOL\xspace}
\newcommand{\inj}{\mbox{\texttt{inj}}\xspace}
\newcommand{\pr}{\mbox{\texttt{pr}}\xspace}


%\usepackage{hetcasl}
%\usepackage{todonotes}


%% Names
\newcommand{\DB}{Dines Bj{\o}rner\xspace}
\newcommand{\Bjoerner}{Bj{\o}rner\xspace}

%% Languages
\newcommand{\CASL}{\textrm{\textsc{Casl}}\xspace}
\newcommand{\ModalCASL}{\textrm{\textsc{ModalCasl}}\xspace}
\newcommand{\RSL}{\textrm{\textsc{RSL}}\xspace}
\newcommand{\MiniDSL}{MiniDSL\xspace}

%% Tools
\newcommand{\Hets}{Hets\xspace}
\newcommand{\Spass}{SPASS\xspace}
\newcommand{\Vampire}{Vampire\xspace}

%% Institutions
\newcommand{\institution}[1]{\mathscr{#1}}
\newcommand{\instSigop}{\mathrm{Sig}}
\newcommand{\instSig}[1]{\instSigop^{\institution{#1}}}
\newcommand{\instModop}{\mathrm{Mod}}
\newcommand{\instMod}[1]{\instModop^{\institution{#1}}}
\newcommand{\instSenop}{\mathit{Sen}}
\newcommand{\instSen}[1]{\instSenop^{\institution{#1}}}
\newcommand{\instmodels}[2][]{\mathrel{\models^{\institution{#2}}_{#1}}}
\newcommand{\instPresop}{\mathrm{Pres}}
\newcommand{\instPres}[1]{\instPresop^{\institution{#1}}}

\newcommand{\ppinstitution}[1]{\institution{\powerset_{*}#1}}
\newcommand{\ppinstMod}[1]{\instMod{\ppinstitution{#1}}}
\newcommand{\ppinstmodels}[2][]{\instmodels[#1]{\ppinstitution{#2}}}

\newcommand{\ppmorphMod}[1]{\rho_{\institution{#1}, \ppinstitution{#1}}^{\instModop}}

\newcommand{\ippinstitution}[1]{\institution{\powerset_{*}^{\mathrm{i}}#1}}
\newcommand{\ippinstSig}[1]{\instSig{\ippinstitution{#1}}}
\newcommand{\ippinstSen}[1]{\instSen{\ippinstitution{#1}}}
\newcommand{\ippinstMod}[1]{\instMod{\ippinstitution{#1}}}
\newcommand{\ippinstmodels}[2][]{\instmodels[#1]{\ippinstitution{#2}}}

\newcommand{\ippinstcomorph}[1]{\mu^{\ippinstitution{#1}, \institution{#1}}}
\newcommand{\ippinstcomorphSig}[1]{\Phi^{\ippinstitution{#1}, \institution{#1}}}
\newcommand{\ippinstcomorphSen}[1]{\alpha^{\ippinstitution{#1}, \institution{#1}}}
\newcommand{\ippinstcomorphMod}[1]{\beta^{\ippinstitution{#1}, \institution{#1}}}

\newcommand{\incppinstitution}[1]{\institution{\powerset_{*}^{\hookrightarrow}#1}}
\newcommand{\incppinstSig}[1]{\instSig{\incppinstitution{#1}}}
\newcommand{\incppinstSen}[1]{\instSen{\incppinstitution{#1}}}
\newcommand{\incppinstMod}[1]{\instMod{\incppinstitution{#1}}}
\newcommand{\incppinstmodels}[2][]{\instmodels[#1]{\incppinstitution{#2}}}


%% Layout
%\parindent0pt
\allowdisplaybreaks
\sloppy


